Neural Databases

In recent years, neural networks have shown impressive performance gains on long-standing AI problems, and in particular, answering queries from natural language text. These advances raise the question of whether they can be extended to a point where we can relax the fundamental assumption of database management, namely, that our data is represented as fields of a pre-defined schema. This paper presents a first step in answering that question. We describe NeuralDB, a database system with no pre-defined schema, in which updates and queries are given in natural language. We develop query processing techniques that build on the primitives offered by the state of the art Natural Language Processing methods. We begin by demonstrating that at the core, recent NLP transformers, powered by pre-trained language models, can answer select-project-join queries if they are given the exact set of relevant facts. However, they cannot scale to non-trivial databases and cannot perform aggregation queries. Based on these findings, we describe a NeuralDB architecture that runs multiple Neural SPJ operators in parallel, each with a set of database sentences that can produce one of the answers to the query. The result of these operators is fed to an aggregation operator if needed. We describe an algorithm that learns how to create the appropriate sets of facts to be fed into each of the Neural SPJ operators. Importantly, this algorithm can be trained by the Neural SPJ operator itself. We experimentally validate the accuracy of NeuralDB and its components, showing that we can answer queries over thousands of sentences with very high accuracy.

==> figures/4_model_comparison.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/model/transformer_comparison_2.pdf}
    \caption{Left: Multiple updates input to transformer model generating multiple answers for query $q$ (prototype). Right: independently generating intermediate fact representation dependent on query.}
    \label{fig:comparison}
\end{figure}

==> figures/4_model_e2e.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figures/model/e2e.pdf}
    \caption{Left: Multiple updates input to transformer model generating multiple answers for query $q$ (prototype). Right: independently generating intermediate fact representation dependent on query.}
    \label{fig:architecture}
\end{figure}

==> figures/6_results_oracle.tex <==
\begin{table}[]

\centering

\begin{tabular}{@{}lc@{}}
\toprule
\textbf{Operation}                          & \textbf{Exact Match (\%)}  \\ \midrule
Question Answering (Atomic)        & $99.2 \pm 0.05$   \\
Question Answering (Explicit Join) & $99.5 \pm 0.4$    \\
ArgMin/ArgMax                      & $92.4 \pm 0.5$    \\
Set                                & $85.0 \pm 2$ (F1) \\
Count                              & $78.5 \pm 0.7$    \\ \bottomrule
\end{tabular}

\caption{Oracle Exact Match scores for variadic T5 model, concatenating facts together for variadic operations. For atomic questions, a single fact is used, for explicit join, a combination of 2 facts are required. For the min/max, set and count operations, a maximum of 50 operands were used.}
\end{table}

==> figures/6_results_retriever.tex <==
\begin{figure}

\centering

\includegraphics[width=\linewidth]{figures/results/t5_tfidf.pdf}

\caption{Model exact match score combining TF-IDF retrieval with Neural Database Variadic T5 Model}
\label{fig:t5:tfidf}
\end{figure}

==> figures/6_results_retriever_bert.tex <==
\begin{figure}

\centering

\includegraphics[width=\linewidth]{figures/results/bert_IR.png}

\caption{Model exact match score combining BM25 or TF-IDF retrieval with a simple question classifier}
\label{fig:bert:tfidf}
\end{figure}

==> figures/binary_classifier.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/binary classifier.pdf}
    \caption{Binary Classifier in SSG}
    \label{fig:binary_classifier}
\end{figure}

==> figures/issg.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/issg_image.pdf}
    \caption{Incremental Set Completion in ISSG}
    \label{fig:issg}
\end{figure}

==> figures/results/ds-ssg.tex <==
\begin{table}[]
\centering
\caption{Performance of SSG trained by distant supervision data by query type} 
\label{ds_issg}
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Query type}} &  \textbf{Precision} & \textbf{Recall}  \\ \midrule
Atomic Boolean                            & 0.8315 & 0.9967                \\
Atomic Extractive                             & 0.8642 & 0.9971          \\
 \midrule
Join Boolean                               & 0.7580               & 0.8799                  \\
Join Extractive                               & 0.8101 & 0.9823               \\
 \midrule
Set                                        & 0.4116 & 0.8822                 \\
Count                                        & 0.6670 & 0.9367                  \\
Arg Min/Max                                         &0.5932 & 1.0               \\ \bottomrule
\end{tabular}
\end{table}

==> figures/results/issg_supervised.tex <==
\begin{table}[]
\centering
\caption{Performance of SSG trained supervised by query type} 
\label{supervised_issg}
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Query type}} &  \textbf{Precision} & \textbf{Recall}  \\ \midrule
Atomic Boolean                            & 0.9723              & 0.9854                 \\
Atomic Extractive                             & 0.9068              & 0.9334                 \\
 \midrule
Join Boolean                               & 0.7356              & 0.9980                  \\
Join Extractive                               & 0.7607               & 0.9794                \\
 \midrule
Set                                        & 0.8803              &  0.9613                 \\
Count                                        & 0.8851              & 0.9596                  \\
Arg Min/Max                                         & 1.00              & 1.00                 \\ \bottomrule
\end{tabular}
\end{table}

==> figures/results/ssg.tex <==
\begin{table}[]
\centering
\caption{Querying the Neural Query Processor from Section~\ref{section:first-experiment} to generate Support Sets for the Neural Query Processor} 

\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Method}} & \textbf{Num} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\ \midrule
Atomic + Joins (top 1)              & 1.0               & 95.62              & 90.39           & 92.93       \\
Atomic + Joins (top 3)              & 3.0               & 36.30              & 97.93           & 52.96       \\
Atomic + Joins (all)                & 11.48             & 8.08               & 99.28           & 14.95       \\ \midrule
Aggregations (top 1)                & 0.6               & 88.86              & 13.59           & 23.57       \\
Aggregations (top 3)                & 1.8               & 74.33              & 21.12           & 32.90       \\
Aggregations (all)                  & 15.74             & 51.63              & 44.16           & 47.61       \\ \midrule
All (top 1)                         & 0.8               & 92.70              & 57.20           & 70.75       \\
All (top 3)                         & 2.5               & 53.73              & 64.75           & 58.12       \\
All (all)                           & 16.2              & 26.90              & 75.47           & 39.66       \\ \bottomrule
\end{tabular}
\end{table}

==> old_2_problem_definition.tex <==
\section{Problem Definition}

\jt{Design choices - could decide on an explicit memory - stored in text vs information stored in langauge model perhaps? Does the brain clude the data or does the brain do the reasonoing with text data. Compare to fabio petroni's paper}


We begin by describing the basic setting of a \ndb, giving a high-level overview, before describing the \ndb architecture in depth. 

The storage media, or \textbf{memory}, of the \ndb\ is an ordered sequence of facts stored as natural language text. A new \ndb\ is initialized with an empty memory. 
The inputs to a \ndb\ are \textbf{facts} and \textbf{queries}: facts modify the state of the memory by appending the text to the memory, without modification of existing facts, and do not return an output; whereas queries return an output without modifying the memory. 
Both the facts and queries input to the \ndb\ are specified as a single sentence natural language utterance. 
The user doesn't have to distinguish between an update or a query because the natural-language processing (NLP) technology can reliably and accurately classify the input. 
While the addition of facts does not modify existing facts in the memory, they may change the model state and answers for specific queries: for example, adding a fact that `{\sc John is unemployed}' would update how the model answers `{\sc What is John's job?}', but not update the answer to the query `{\sc What jobs has John had?}'.
Using this state update mechanism the model can also support deletions through invalidating stored facts. 

\input{figures/2_example.tex}

\subsection{NeuralDB Interface}
Let $D$ be an ordered database of facts stored in free-form natural language text without a schema $(d_1,\ldots,d_k)$.
The \ndb\ is two composed of two functions $f: (x,D) \to y$ yielding an answer $y$ to natural language query $x$ and $g: (x,D) \to D'$, appending fact $x$ to the memory: $D' = D \frown (x)$. The query or update function, $f$ or $g$ respectively, is selected through classification of the input $h: x \to \{f,g\}$.


\subsection{Storing Facts}
Updates to the database are stored as natural language text.
In this work, we assume the unique names assumption; this means we assume that a name exactly refers to a single entity mentioned in the database. 
The application of the rich body of work on entity resolution to \ndb s will be reserved for future work. 
Despite this, we show that \ndb s are capable of handling a range of expressions: in Section~\ref{section:experiments:alias} we will demonstrate that aliases for entities and properties can be resolved using parametric information captured within pre-trained language models.

Even though updates are always single sentences specified in natural language, we distinguish atomic updates from composite ones. 
Atomic updates are meant to express one fact, e.g., {\sf Sue is Mary's mom}, or {\sf Gustavo likes espresso}. 
Composite updates are sentences that may encode multiple facts, e.g., {\sf Kanesha is married to Kyrone and they have 3 kids}. 
We imagine that in the applications that \ndb s are meant to support, users will find it more natural to express composite updates. 
In Section~\ref{section:experiments:composite} we describe experiments with both atomic and composite updates. 


\subsection{Querying the NeuralDB}
\jt{class of queries - what works / what doesn't work}
At query time, the model performs a computation over relevant facts $Z \subseteq D$; without explicit supervision as to which facts are needed to compose an answer to the query. 
The model must support a number of operations that combine and aggregate information from these facts: some require language understanding, such as Boolean question answering: {\sf Does Gustavo like espresso?} and others require mathematical reasoning: {\sf Who has the most children?}.
In this paper we consider the following operators: {\tt argmin/max}, {\tt min/max}, {\tt count} set cardinality, return a {\tt set}, and {\tt Boolean} question answering. All of these must execute on queries which operate both on atomic facts as well as compositions of facts: our model of a natural join.

To execute a query, the \ndb\ requires a program of operators which transform the stored data into the output. These are broken into three classes: unary, binary and variadic operators.

\noindent{\bf Unary operators:} analogous to {\em select}, {\em project} and {\em rename} in relational algebra, we introduce a Neural Unary Operator (NUO; $\upsilon$) that performs a conditional transformation on facts independently, dependent on the query: $\upsilon_{x} (D)=\{\upsilon_x(\{d_i\}) | d_i \in D\}$. 
This operator performs both a high-precision selection operation, filtering out irrelevant facts as well as rewriting the sentence to an intermediate form suitable for downstream operators. 
For composite updates that express multiple facts, this operator will select a subset of these, for those needed to answer the query.

% Not yet tested - but would be cool to do if there is time.
\noindent{\bf Binary operators:} supporting natural joins requires a binary operator. We posit that a recurrence over the unary operator would suffice $Z^{(t+1)} = \upsilon_{x, Z^{(t)}}(D)$. Concretely, this would conditionally encode each fact $d_i\in D$ dependent on the query and the data in a recurrence memory, forming a composite fact. Each step in a multi-hop join is one application of the operator. 

\noindent{\bf Variadic operators} the \ndb\ must combine a varying number of facts to aggregate information. This computation could either be neural, performing a {\tt Boolean} question answering task over multiple retrieved sentences, or use classical computation for mathematical reasoning problems such as {\tt counting} and {\tt argmax}. The choice of variadic operator would depend on classification of the query, while it would be an exciting proposition to perform all numerical reasoning within a neural model, we show that the limited numerical reasoning ability of neural model precludes direct application.

For neural reasoning over text, there are two ways in which information can be composed: concatenation of texts and fusion in decoder \cite{Izacard2020}. For concatenation of texts, this operator `understands' composition of facts as the input string is encoded with self-attention. 
We demonstrate a baseline \ndb\ architecture using only a single variadic neural model in Section~\ref{section:experiments:baseline} that works for small databases. 
However, this has a fundamental limitation that would prevent it from scaling to large databases because of the number of texts that can be encoded: as these neural models rely on self-attention, that has quadratic complexity, it is not feasible to encode sequences longer than 1000 tokens. 
Fusion-in-decoder is a workaround where sentences are independently encoded and combined when generating an output; we show experimentally that self-attention between facts is required for composition in Section~\ref{section:experiments:fusion}. 

\subsection{World Knowledge vs Explicit Join}
For both the unary and variadic neural components, we fine-tune networks derived from pre-trained Language Models (LM). \jt{we use BERT/T5 LMs for our task \todocite{Raffle2020}}
LM pre-training embeds world knowledge within the model parameters, capturing a number of facts and common sense implicitly \cite{Petroni2019} that mitigate the need for explicit joins for some queries.
We show the pre-training is essential for building \ndb s that scale to a broad range of topics through ablation experiments in Section~\ref{section:experiments:lm}.

\jt{Where should implicit/explicit knowledge lie? How can this help us \cite{Clark2020,Talmor2020}}



==> old_3_model.tex <==
\section{Model}
\ndb\ is an architecture that allows facts stored in natural language to be queried with natural language.
The core component of this are neural network models that encodes text and conditionally transduces it, decoding a different string. 
This class of model is an encoder-decoder and has been applied to numerous settings, including machine translation and document summarization.

The composition of the models with information retrieval is gives the behaviour of the neural database.
While the variadic and unary operators use the same model architecture, they are trained with different data to have different behaviours.

\subsection{Variadic operator}
The variadic model (Figure~\ref{fig:model:variadic}) takes in an unspecified number of facts - from zero or more - in combination with the query and performs neural reasoning outputting a string. There are two approaches for this: either concatenating the sentences together and encoding, or separately encoding the facts. 

We could potentially encode the entire database as a single input to this variadic model: however, the self-attention mechanism within the transformer model architecture has a quadratic complexity which precludes this model architecture from scaling to very large databases. Furthermore, as numerical reasoning capabilities in neural networks are limited, this model could not scale to answer queries which require numerical computation.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/model/variadic_example.pdf}
    \caption{Variadic neural reasoning with a transformer model, concatenating the query with facts}
    \label{fig:model:variadic}
\end{figure}



\subsection{Unary operator}
The unary operator (Figure~\ref{fig:model:unary}) inputs a single fact and conditionally projects it to a different string dependent on the query. For example, for a query which performs an argmax over records, the operator projects the fact to a tuple containing the entity name and a numeric value. This allows aggregations and computations over many facts to be computed through classical computation, overcoming limitations of the transformer model which is unable to encode long strings and has limited numerical reasoning capability.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/model/unary_operator.pdf}
    \caption{Unary neural reasoning with a transformer model, generating an appropriate structured intermediate representation of the facts to perform numerical aggregation with classical computation}
    \label{fig:model:unary}
\end{figure}

With the exception for queries requiring set-based answers, the unary operator needs to be combined with another aggregation module to return an answer. We propose using {\em classical} aggregation functions for numerical operations such as argmin, argmax, counting the cardinality of a set etc selected depending on the type of question, and using {\em neural} aggregation, such as the variadic question answering model, for queries requiring natural language understanding.

The unary operator is used to perform both a high precision selection depending on the query as well as performing a query-dependent projection. For facts that do not contain relevant information that can be used to answer the query, the model should project the fact to a null token that will be filtered. 

\subsubsection{Performing joins using a conditional encoding in the unary operator}
\jt{I'm not sure if there's maybe time or space for this yet. But what I'd like to perhaps look at is whether we can perform joins within this unary operator in an iterative manner through applications of the operator, conditionally encoding the facts in the database with the query as well as previously selected information from the previous time step.}

\subsection{NDB Architecture}
The \ndb\ architecture we present is an ensemble of the unary and variadic operators. The unary operator performs a high-precision selection and projection of the facts in the database to an intermediate form, we select an aggregation function dependent on the query. The architecture diagram in Figure~\ref{fig:model:architecture} shows the following (from left to right): (1) combination between every fact in the database and the query, input into the unary operator (2) the unary operator either performing high precision selection of the (query, fact) tuple or performing a projection dependent on the query type (3) the query is classified and used to select an aggregation function, for example, queries requiring an argmax would select a classical implementation of an argmax operation whereas queries requiring natural language reasoning would use a variadic neural model to ansewr the query (4) application of an appropriate variadic aggregation function where needed or returning a set of facts (e.g. for a `list all' type query).

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/model/architecture.pdf}
    \caption{End-to-end neural database architecture showing data flow between the operators to generate an answer to a query. Thick arrows represent a multi-set of of items, thin arrows represent a single item. }
    \label{fig:model:architecture}
\end{figure}





\subsection{Implementation}

\noindent{\textbf{NN Architecture: }} The \ndb\ models use transformer neural network architecture \cite{Vaswani2017} which uses self-attention to generate contextual representations of tokens: mapping a word in context to a real-valued vector of fixed dimension.
The model is trained with supervision to incrementally predict tokens, to decode the output string. 
The supervision comes from curated sentence pairs of inputs and outputs: errors made when decoding the output are used to update the model parameters.

\noindent{\textbf{NN Pre-training: }} The value of transformer models is that their efficient architecture allows scaling training to corpora of billions of tokens. Using a Language Modelling (LM) training objective, world knowledge can be embedded into the model parameters with relatively low cost as there is an abundance of data to supervise training. The supervision for LM pre-training comes from unlabelled sentences, with tokens randomly masked that the model has to predict the missing word for (see BERT/T5 \cite{Devlin2019, Raffel2020}).

% model configuration file: https://s3.amazonaws.com/models.huggingface.co/bert/t5-base-config.json
\jt{Implemented using HuggingFace, use a T5-base model 12 layers, 12 heads, 768 dimension representation}


==> old_3_training.tex <==
\section{Training a \neurodb} 
\label{training}

* Recurrent neural network architectures are used for numerous sequence transduction tasks \citetodo{Graves2012}: e.g. speech recognition, machine translation, parsing text into queries.

* These models are trained in a supervised setting: the models are trained with examples of what the output should be. For example, in machine translation, translating english to french, both the english and french sentences are given. 

* At the heart of the neural database is a string transducer that takes a set of facts, stored in natural language, in a database that outputs a string containing the answer to a given query.

* The model we use is a T5 transformer \citetodo{Raffel2019}, a transformer model that is pre-trained using unlabelled data. This model is trained to predict the most likely missing tokens masked from web pages. The model is pre-trained using the C4 common crawl dataset  which is two orders of magnitude larger than Wikipedia. This allows it to be fine-tuned on a specific task, such as the \neurodb task with relatively fewer training examples. 

* In this paper, we experiment with two topologies for \neurodb: the first is a variadic encoder model where database facts are encoded by a single model (either jointly or in isolation) to synthesize an answer. The second topology is a unary operator which jointly acts as a high precision selection and projection function that encodes each fact in isolation into an intermediate string representation depending on the query.

* we show, experimentally that these two topologies are complementary: the variadic model has a very good ability to understand natural language and compose multiple facts together allowing us to perform joins and that  multiple facts together   behavior. the 





We have multiple components in our architecture, depending on how we train these components, we can divide our training strategy into two broad categories:


\paragraph{End2end training}
Each training example in \ndb is a tuple $((u_1 \cdots u_t), q , a)$ in which \textit{q} is a query, \textit{a} is an answer, and $(u_1 \cdots u_t)$ is all the updates in the database before the query is asked. In this case, all the components are trained such that for every question, the right answer is found. The main issue is that the output of the neural retriever and unary neural operator components are discrete symbols, and we need to train them to output discrete latent variables that are useful in finding the right answer. End2end training needs marginalizing over these latent discrete variables using an approximation algorithm or reinforcement learning algorithms.  (More details when we figured the right algorithm)


\paragraph{Component-wise}
In this case, we train each component in isolation and put them together at the inference time. We need to gather training data for each component separately: we should know the correct intermediate symbolic representations for each component. Each component that is trained independently gives us a great starting point for an end2end training that alleviates brittleness of cold start in end2end training.

==> old_6_results.tex <==
\section{Results}

\subsection{Variadic Models}
\label{section:experiment:baseline}


First we check the ability of the T5 model to perform variadic combination of facts for question answering. We evaluate two variants of the T5 model that consider concatenation of facts and through using fusion in decoder.

\subsubsection{Oracle Model}
We consider an oracle environment where only the relevant facts are input to the model. We use a sample dataset of generated facts and queries that are a synthetic combination of real-world entities over 16 relations. For variadic operations, such as {\tt argmax} and {\tt count}, we consider cases which require less than 50 operands. 

The model attains near-perfect accuracy for question answering type queries where either a single fact is needed, or where a composition over pair of facts is needed to answer the query. The model has lower accuracy for tasks generating a set of answers and for counting. This can be due to limitations in numerical reasoning and conditional decoding.

\input{figures/6_results_oracle}

There is a fundamental limitation with the transformer model as there number of input tokens and output tokens are finite, this prevents large contexts from being joined together for variadic question answering, and from the entire database from being encoded for question answering. 
This is demonstrated in the oracle environment by increasing the the number of operands for variadic operations from $50$ to $100$. While accuracy for question answering remains unchanged, {\tt set} answer EM drops to $65.7\%$, {\tt count} EM drops to $52.1\%$ and {\tt argmin/argmax} drops to $68.0\%$.

\subsubsection{Small database model}
\jt{Putting the entire database as context} 


\subsubsection{Large database model: Combining Information Retrieval}
In practice the input size for the transformer is limited to 256, 512 or 1024 tokens. This limitation precludes its use for queries which require reasoning over a large number of updates. Runtime complexity is quadratic w.r.t sequence length for both input and output strings. %Furthermore, numerical reasoning capabilities in neural networks are limited and need to be better studied.

To scale the neural database to large databases, we incorporate information retrieval with the variadic reasoning model. We consider three types of IR model: BM25, TF-IDF and neural information retrieval models. Figure~\ref{fig:bert:tfidf} Simple model: considers neural databases as a classification task, compare BM25 and TF-IDF. TF-IDF works better than TF-IDF - BM25 issues: is the sparsity penalty of BM25 causing a problem?
\jt{TODO: show precision and recall for the information retrieval components}
\input{figures/6_results_retriever_bert}


Figure~\ref{fig:t5:tfidf} uses T5-IDF as a retriever: for question answering and queries with a single answer, the model attains near perfect accuracy for smaller databases. For larger databases with more complex queries (aggregations and sets), the peak accuracy is lower, but does not decrease as a function of database size.

\input{figures/6_results_retriever}

\jt{The accuracy for queries requiring joins or aggregations is lower than the oracle environment: losing recall for the joined data - not returned from TF-IDF sometimes because there is no joined information}


\subsubsection{Math reasoning}
\jt{Could perhaps state how the model struggles with argmin/argmax queries in a math world setting - a bit more fine-grained than Marzieh's data}


\subsubsection{Cross-domain relation transfer}
We train the model ommiting some queries without 


\subsubsection{Memorization vs Understanding}

\subsubsection{Susceptibility to Noise}
Adding 

\subsection{Unary Operators}
Consider the unary operator in isolation.

\jt{Will it project a fact to a query}


\subsubsection{Cross-domain relation trasnfer}
\subsubsection{Entity resolution}




==> oldstuff.tex <==
\medskip
\noindent
{\bf Data categories: (OLD STUFF)}
\begin{itemize}
    \item [D1:] Data is stated in single facts in a particular domain. (e.g., {\em Mark lives in London})
    \item [D2:] Data is stated in phrases that may contain multiple facts. (e.g., {\em Mark lives in London with his wife})
    \item [D3:] D2 + data may include facts that use relations from "world knowledge". For now, let's make the convenient assumption that world knowledge is the facts that use predicates from Freebase and its equivalents. 
    \item [D4:] Data can be about any domain.
\end{itemize}



Let's consider data of type D1 for the following analysis. The different categories of queries suggest (a) the different components in our system and (b) which training data we should attempt to collect.

Below we identify four classes of \neurodb\s (with affectionate and temporary  names). Please note that the categories defined by Q1-Q3 above are rather coarse and are designed so these classes can be defined. 

\medskip
\noindent{\bf Bear bones DB:}
Consider the base case, queries of type Q0. This is the bare bones \neurodb. The goal of this database is to not do anything stupid. So one issue we identified already is not to {\em forget}. Specifically, if I told you fact $f_1$ and then gave you any number of other facts (not related to $f_1$), then if I query $f_1$, the answer should be True (or if the query had a variable in it, then it should be the value in $f_1$). There are likely other issues that may arise which we don't know yet. We should create testing data sets to endow the \neurodb\ with this capability. 

\medskip
\noindent{\bf Language agnostic lookup:} In this case we consider Q1 queries (but still D1 data). Queries can be formulated naturally (which means that the facts can be formulated naturally too). We're hoping that the pre-trained language model (plus additional corpora for the domain) may give us what we need here, but we also need (query, answer) pairs so the system is smart enough to recognize query forms. Perhaps there is a good resource for such pairs (or perhaps there's a fast way to bootstrap them for a domain).  

\medskip
\noindent{\bf The neural reasoner:} Now we're considering Q2 queries. The challenge here is to learn the possible reasoning paths we may need to answer queries. These paths can be special to a domain, but some of them come from what we call world knowledge (which we'll think of as Freebase+Geo+Time reasoning). 

We have a component in our system design that decides whether to try to go one more step to find an answer to a query. Note that sometimes we may have partial answers after a smaller number of steps. For example, for Joe's uncles, I may have a fact that tells me that George is Joe's uncle, but for other uncles I may have to traverse parent-brother paths (or even grandparent-son paths). 

Intuitively, it seems like these paths themselves can be stored in some new form of a pre-trained model (i.e., a pre-trained models for paths). In fact, that pre-trained model can be a contribution in itself that can be used in other places. In fact, we can think of these paths as sequence-to-sequence transformations (e.g., the sequence \{uncle, father\} would be extended by brother, and the sequence \{uncle, grandmother\} would be extended by son). Note that the query term is the first element of the sequence (which is a simple case, some queries will need richer representations). Of course, the tokens in these sequences are merely place holders for atomic queries because the token grandmother may be stated in many ways in the data. But at least this formulation puts us back into known neuro land. Another difference to keep in mind is that we need to follow multiple sequences, not just one as one would do in machine translation, for example. 

\medskip
\noindent{\bf The database cherry on the cake:} Now we consider Q4 queries. How do we do aggregation? That probably requires another component in the system that we may not have yet. Some inspiration from Neural Turing machines may be useful. 

\section{\neurodb\ architecture}
This section explains the principles of a neural database.

Basic idea: the system has a memory and an inference engine. What happens in training time and query time. 
\subsubsection*{Intuition} First we need to explain the intuition underlying the \neurodb. Specifically, what is the system learning? 

Ideally, the system would learn some of the items below. The point of this paper is to explore which of these it can learn and supplement the system with additional operators to answer more complex queries. 

\begin{itemize}
    \item Lookups that are independent of linguistic form:  The basic operation of a database system is to look facts up. \neurodb\  learns linguistic variations (which it essentially gets from Roberta). As an example, the system would know that {\em Mike is Susan's father} states the same fact as {\em Susan's dad is Mike}. This means that we can retrieve facts without knowing exactly how they were given to the database. This is a huge advance from existing database systems. 
    \majidquestion{I believe we need more than what a language model like RoBERTa can provide. But, transformers LMs are good starting point. We need co-reference, entity and relation extraction (it might be done implicitly not explicitly), disambiguation and etc. These are not supported in the best way by LM loss.}
    \item Database operations: \neurodb\ learns how to perform basic database operations: (which it gets from an internal component in the architecture of \neurodb). As an example, it learns how to do a join (most likely, a linear join which is similar to following a path in a graph). The system can also learn how to perform selections (e.g., {\em find all kids younger than 15}), and maybe how to aggregate (e.g., {\em how many kids does Mary have?}). It's likely that the first version of \neurodb\ won't be able to do all of these.
    \majidquestion{I see two scenarios: 1- these operations are neural(embedded in NN parameters) 2- these are hard-coded functions that \neurodb\ learns to call, any pros-cons?}
    \item Domain knowledge: we can also train a \neurodb\ to understand more knowledge about the domain of the application. For example, if the database is about sports, then we can further specialize the training corpus with texts about sports, and then the system would know that BA stands for batting average and that the superbowl is the final and deciding game of a football season. It could also know about specific players in each sport and the teams they played for.
    \item World knowledge: \neurodb\ can leverage existing bodies of knowledge (e.g., Wikipedia) to answer more complex queries or perform some simple common-sense reasoning. For example, \neurodb\ can know that London is in England. Hence, if I tell it that Mike lives in London, then the answer to the query {\em friends living in England} will include Mike. It is important to note that \neurodb\ {\em does not} achieve this by doing a join! It achieves this by,.. well, we don't exactly know! It's part of the magic of the neural inference. Note that the distinction between domain knowledge and world knowledge is not a clear one. 
    
\end{itemize}

Given that we clarified the intuition about what the database is learning, we can now describe the architecture in more detail and the training process and training data.

The description of the architecture should have boxes for pre and post processing. The questions here are what are the most important ways we can help the neural machinery achieve the database goals:

\begin{itemize}
    \item On updates: should we break down updates to their individual components (e.g, entities, relationships) before we give them to the \neurodb? The paper should examine whether there is a benefit in doing so.
    \majidquestion{does this mean doing IE on the updates first?}
    \item On queries: it's likely that the first version of \neurodb\ won't be able to answer arbitrary SQL queries. The question is what operators can the system learn? The post-processing will complement these operators with traditional database processing. Possible answers to this question are: 
    \begin{itemize}
        \item \neurodb\ supports only retrieval -- everything else has to be done relationally. That's still great.
        \item Can \neurodb\ answer non-ground queries? e.g., friends living in London (in DB notation: Lives(X, London))
        \item \neurodb\ does retrieval but then applies world knowledge along the way. So I get that Mike lives in England. 
        \item \neurodb\ can follow N edges in a join graph (and increasing N just means giving more training data or changing the architecture in some generic way). 
        \item \neurodb\ also learns common views. For example, if I asked it for all of the children, and it was told that Joe is 15, then Joe will be in the answer. In this case, \neurodb\ is using {\em schematic} world knowledge that people younger than 18 are kids and applying this knowledge to the query. This is a bit more sophisticated than understanding different linguistic patterns because there is some inference there that in database language amounts to a view and to answering queries using views~\cite{DBLP:journals/vldb/Halevy01}.
        \majidquestion{what is the difference between this and common-sense reasoning?}
    \end{itemize} 
\end{itemize}

\eat{
Queries may require some path traversal/reasoning: 
    \begin{itemize}
        \item {\em Who is Sam's uncle?} May need to be composed from two facts: Liz is Sam's mother and George is Liz's brother.
        \item {\em Is Jill a child?} May need to be composed of Jill is 15 years old, anyone under 18 is a child. 
        \item {\em How old is Jill?} May need to be composed of Jill is a child, children are younger than 18 (hence, the answer is: under 18).
        \item Does Grace live in London? May need to be composed of Grace moved to London and the commonsense knowledge that says that when you move somewhere you live there. 
        \end{itemize}
        
        
\begin{itemize}
    \item [Q0:] Queries are lookups. The query is formulated exactly like a fact (e.g., {\em joe is the father of sue}). (Note that database query languages essentially formulate queries as facts). 
    \item [Q1:] Queries are still atomic (i.e., the answer, if it exists, is in the database as a single fact), but the query can be formulated more naturally (e.g., {\em who is Sue's father}). Note that to answer these kinds of queries we need some paraphrasing capabilities.
    
    \item [Q2:] Queries may require some path traversal/reasoning: 
    \begin{itemize}
        \item {\em Who is Sam's uncle?} May need to be composed from two facts: Liz is Sam's mother and George is Liz's brother.
        \item {\em Is Jill a child?} May need to be composed of Jill is 15 years old, anyone under 18 is a child. 
        \item {\em How old is Jill?} May need to be composed of Jill is a child, children are younger than 18 (hence, the answer is: under 18).
        \item Does Grace live in London? May need to be composed of Grace moved to London and the commonsense knowledge that says that when you move somewhere you live there. 
    \end{itemize}
    \item 
\end{itemize}
}


At training time, the system is given updates and queries. These updates and queries are in the same domain as the application for which we're building the database but they will be about different entities. \alonquestion{How do we guarantee that the data instances are not carried over from the training to the application? For example, in the training data I may have said that Susan's mom is Julie, but in my specific database instance I should not get Susan as Julie's mom.}
\majidquestion{I think fundamentally we have two approaches: 1- train it not doing that (a.k.a there is a loss function penalizes such thing) 2- add something in the architecture to prevent that  ... or both}
